H2O Southern Galactic Plane Survey (HOPS): Paper III - Properties of Dense Molecular Gas across the Inner Milky Way

The H2O Southern Galactic Plane Survey (HOPS) has mapped 100 square degrees of the Galactic plane for water masers and thermal molecular line emission using the 22-m Mopra telescope. We describe the automated spectral-line fitting pipelines used to determine the properties of emission detected in HOPS datacubes, and use these to derive the physical and kinematic properties of gas in the survey. A combination of the angular resolution, sensitivity, velocity resolution and high critical density of lines targeted make the HOPS data cubes ideally suited to finding precursor clouds to the most massive and dense stellar clusters in the Galaxy. We compile a list of the most massive HOPS ammonia regions and investigate whether any may be young massive cluster progenitor gas clouds. HOPS is also ideally suited to trace the flows of dense gas in the Galactic Centre. We find the kinematic structure of gas within the inner 500pc of the Galaxy is consistent with recent predictions for the dynamical evolution of gas flows in the centre of the Milky Way. We confirm a recent finding that the dense gas in the inner 100pc has an oscillatory kinematic structure with characteristic length scale of ~20pc, and also identify similar oscillatory kinematic structure in the gas at radii larger than 100pc. Finally, we make all of the above fits and the remaining HOPS data cubes across the 100 square degrees of the survey available to the community.

==> tables/derivs.tex <==
\begin{tabular}{|r|r|r|r|r|r|l|}
\hline
  \multicolumn{1}{|c|}{lCent\_deg} &
  \multicolumn{1}{c|}{bCent\_deg} &
  \multicolumn{1}{c|}{T\_rot\_K} &
  \multicolumn{1}{c|}{N\_nh3\_tot} &
  \multicolumn{1}{c|}{T\_kin\_K} &
  \multicolumn{1}{c|}{fwhm\_nt} &
  \multicolumn{1}{c|}{fwhm\_th} \\
\hline
  29.9386 & -0.03095 & 19.0 & 1.69 & 22.0 & 3.13 & 0.24\\
  27.77443 & 0.06791 & 21.0 & 0.69 & 26.0 & 2.37 & 0.26\\
  27.27837 & 0.15187 & 42.0 & 0.45 & 93.0 & 2.32 & 0.50\\
  24.78522 & 0.09488 & 17.0 & 2.22 & 20.0 & 3.58 & 0.23\\
  24.47508 & 0.47827 & 34.0 & 0.33 & 59.0 & 3.04 & 0.39\\
  24.42476 & -0.21978 & 19.0 & 1.86 & 23.0 & 3.27 & 0.25\\
  18.85464 & -0.47798 & 19.0 & 1.15 & 23.0 & 2.7 & 0.24\\
  14.70352 & -0.1744 & 16.0 & 0.83 & 18.0 & 1.43 & 0.22\\
  14.21368 & -0.48907 & 27.0 & 0.33 & 38.0 & 0.7 & 0.32\\
  14.21031 & -0.18499 & 18.0 & 1.35 & 22.0 & 2.49 & 0.24\\
  13.31567 & -0.29872 & 17.0 & 1.45 & 19.0 & 1.95 & 0.23\\
  13.20766 & 0.05092 & 17.0 & 1.51 & 20.0 & 2.41 & 0.23\\
  12.90054 & 0.48707 & 25.0 & 0.06 & 33.0 & 0.47 & 0.30\\
  10.47778 & 0.03467 & 22.0 & 1.6 & 28.0 & 4.63 & 0.27\\
  9.62135 & 0.18733 & 18.0 & 1.29 & 21.0 & 3.28 & 0.24\\
  9.23748 & -0.18991 & 17.0 & 1.25 & 19.0 & 1.81 & 0.23\\
  8.83139 & -0.03632 & 18.0 & 1.0 & 22.0 & 2.11 & 0.24\\
  8.62073 & -0.34643 & 15.0 & 1.63 & 17.0 & 2.31 & 0.21\\
  7.33549 & -0.00895 & 18.0 & 0.53 & 21.0 & 1.59 & 0.23\\
  6.8806 & -0.24195 & 14.0 & 1.74 & 16.0 & 2.39 & 0.21\\
  6.19456 & -0.36807 & 17.0 & 1.69 & 19.0 & 3.03 & 0.23\\
  5.64038 & 0.23879 & 16.0 & 1.01 & 18.0 & 1.56 & 0.22\\
  3.4476 & 0.00789 & 17.0 & 0.67 & 20.0 & 1.51 & 0.23\\
  3.43198 & -0.35111 & 14.0 & 2.84 & 16.0 & 2.99 & 0.20\\
  1.37351 & 0.11181 & 27.0 & 0.16 & 39.0 & 0.46 & 0.32\\
  0.6578 & -0.2132 & 26.0 & 0.03 & 35.0 & 0.51 & 0.31\\
  359.71081 & -0.37799 & 22.0 & 0.19 & 29.0 & 0.92 & 0.28\\
  359.47531 & -0.03431 & 22.0 & 0.02 & 28.0 & 0.35 & 0.27\\
  359.30111 & 0.03486 & 32.0 & 0.37 & 54.0 & 0.57 & 0.38\\
  355.26149 & -0.25966 & 26.0 & 0.52 & 37.0 & 1.2 & 0.31\\
  353.39238 & -0.34255 & 16.0 & 3.97 & 18.0 & 4.01 & 0.22\\
  353.19352 & -0.23902 & 29.0 & 0.04 & 45.0 & 0.26 & 0.34\\
  352.05378 & -0.2515 & 22.0 & 0.49 & 28.0 & 1.57 & 0.27\\
  351.80157 & -0.45979 & 16.0 & 1.8 & 19.0 & 2.1 & 0.22\\
  351.58024 & -0.34699 & 19.0 & 2.53 & 23.0 & 4.24 & 0.25\\
  349.91123 & 0.08303 & 24.0 & 0.68 & 33.0 & 2.9 & 0.29\\
  348.24932 & 0.4603 & 16.0 & 1.28 & 18.0 & 2.06 & 0.22\\
  345.48768 & 0.3423 & 18.0 & 0.91 & 22.0 & 2.33 & 0.24\\
  345.02635 & -0.21775 & 18.0 & 2.27 & 21.0 & 4.14 & 0.24\\
  344.42507 & 0.0502 & 19.0 & 1.15 & 23.0 & 2.64 & 0.25\\
  341.93617 & -0.17089 & 16.0 & 2.2 & 18.0 & 3.33 & 0.22\\
  340.30222 & -0.37643 & 16.0 & 2.19 & 19.0 & 2.78 & 0.22\\
  340.23864 & -0.03446 & 20.0 & 1.51 & 24.0 & 3.64 & 0.25\\
  338.92434 & 0.38773 & 23.0 & 0.26 & 29.0 & 0.92 & 0.28\\
  338.3813 & -0.41393 & 19.0 & 0.28 & 24.0 & 1.64 & 0.25\\
  337.90932 & -0.46163 & 20.0 & 0.53 & 25.0 & 2.84 & 0.26\\
  337.77417 & -0.33648 & 17.0 & 1.43 & 19.0 & 2.28 & 0.23\\
  336.98506 & -0.01714 & 24.0 & 0.22 & 33.0 & 0.49 & 0.29\\
  336.37033 & -0.00224 & 23.0 & 0.94 & 31.0 & 2.82 & 0.29\\
  335.58784 & -0.28356 & 19.0 & 1.52 & 23.0 & 3.48 & 0.24\\
  335.28004 & -0.12317 & 20.0 & 0.6 & 24.0 & 1.81 & 0.25\\
  333.18255 & -0.40536 & 18.0 & 2.33 & 22.0 & 3.16 & 0.24\\
  331.49066 & -0.10863 & 16.0 & 3.26 & 18.0 & 4.32 & 0.22\\
  331.35942 & 0.16159 & 18.0 & 0.67 & 22.0 & 1.61 & 0.24\\
  330.88096 & -0.37106 & 24.0 & 1.09 & 33.0 & 3.77 & 0.30\\
  329.03271 & -0.1896 & 19.0 & 2.33 & 23.0 & 3.24 & 0.25\\
  327.7215 & -0.38292 & 19.0 & 0.49 & 24.0 & 2.6 & 0.25\\
  326.99614 & -0.03667 & 23.0 & 0.94 & 30.0 & 2.22 & 0.28\\
  318.78338 & -0.13118 & 14.0 & 1.72 & 15.0 & 2.71 & 0.20\\
  317.38856 & 0.11877 & 24.0 & 0.07 & 33.0 & 0.36 & 0.29\\
  316.75237 & 0.00384 & 20.0 & 2.12 & 25.0 & 3.26 & 0.26\\
  310.65968 & -0.2262 & 25.0 & 1.04 & 35.0 & 3.34 & 0.30\\
  305.37698 & 0.21314 & 22.0 & 0.08 & 29.0 & 0.52 & 0.27\\
  305.2308 & 0.27918 & 17.0 & 1.19 & 20.0 & 2.95 & 0.23\\
\hline\end{tabular}

